"Killing Me" Is Not a Spoiler: Spoiler Detection Model using Graph Neural Networks with Dependency Relation-Aware Attention Mechanism

Several machine learning-based spoiler detection models have been proposed recently to protect users from spoilers on review websites. Although dependency relations between context words are important for detecting spoilers, current attention-based spoiler detection models are insufficient for utilizing dependency relations. To address this problem, we propose a new spoiler detection model called SDGNN that is based on syntax-aware graph neural networks. In the experiments on two real-world benchmark datasets, we show that our SDGNN outperforms the existing spoiler detection models.

==> Figures/Figure_2.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{Figures/Figure_2.pdf}
\caption{Architecture of SDGNN}
\label{fig:fig_2}
\end{figure*}
